Channel-driven Decentralized Bayesian Federated Learning for Trustworthy Decision Making in D2D Networks

Bayesian Federated Learning (FL) offers a principled framework to account for the uncertainty caused by limitations in the data available at the nodes implementing collaborative training. In Bayesian FL, nodes exchange information about local posterior distributions over the model parameters space. This paper focuses on Bayesian FL implemented in a device-to-device (D2D) network via Decentralized Stochastic Gradient Langevin Dynamics (DSGLD), a recently introduced gradient-based Markov Chain Monte Carlo (MCMC) method. Based on the observation that DSGLD applies random Gaussian perturbations of model parameters, we propose to leverage channel noise on the D2D links as a mechanism for MCMC sampling. The proposed approach is compared against a conventional implementation of frequentist FL based on compression and digital transmission, highlighting advantages and limitations.

==> sections/d-sgld.tex <==
\section{Decentralized Wireless Federated Langevin Monte Carlo}
\label{sec:d-sgld}

\subsection{Communication Model}

\textcolor{red}{here should add the channel model, shadowing and slot-based communication}

%\textcolor{red}{introduce the full duplex constraint}
The agents are assumed to communicate over full-duplex flat-fading channels where the channels coefficients remain constant throughout the overall communication block and may vary across successive blocks, possibly in a correlated way.  
%We assume block flat-fading channels, where the channels coefficients remain constant throughout the overall communication block and may vary over successive blocks, possibly in a correlated way. 
Each block contains $m$ channel uses, allowing the transmission of the local samples by a device. 
We focus on a non-orthogonal multiple access (NOMA) transmission strategy that can exploit the superposition property of the wireless channel to allow all neighbors of agent $k$ to transmit simultaneously their samples in a single block of $m$ channel uses.  
%, namely orthogonal multiple access (OMA) and non orthogonal multiple access (NOMA).
The latter can exploit the superposition property of the wireless channel to allow all neighbors of agent $k$ to transmit simultaneously their samples in a single block of $m$ channel uses, while OMA requires a larger number of blocks in order to ensure interference-free transmissions, see Sec. ?? where we will discuss the adopted scheduling strategy. 
an additional $(|\mathcal{N}_k| - 1) \cdot m$ number of channel uses to let all neighbors of $k$ transmit their samples. 
For OMA, the individual signals received from the neighbors of agent $k$ are expressed as
\begin{equation}
    \mathbf{y}_{kj}^{[s]} = h_{kj}^{[s]} \mathbf{x}_j^{[s]} + \mathbf{z}_j^{[s]} \qquad \forall_{j} \in \mathcal{N}_{\overline{k}} \qquad \mathrm{(OMA)} \label{eq:oma_signal}
\end{equation}
where is the channel gain between agent $k$ and $j$ in round $s$, $\mathbf{x}_{j}^{[s]}$ is an uncoded function of the \textcolor{black}{local samples $\boldsymbol\theta_j^{[s]}$} and $\mathbf{z}_{j}^{[s]} \sim \mathcal{N}(0, N_0 \mathbf{I}_{m})$ is the Gaussian i.i.d. channel noise. 
the received signal at agent $k$ for the $s$-th communication round is
\begin{equation}
    \mathbf{y}_{k}^{[s]} = \sum_{j \in \mathcal{N}_k} w_{kj} (h_{kj}^{[s]} \mathbf{x}_{j}^{[s]} + \mathbf{z}_{kj}^{[s]}) = \sum_{j \in \mathcal{N}_k} w_{kj} h_{kj}^{[s]} \mathbf{x}_{j}^{[s]} + \sum_{j \in \mathcal{N}_k} w_{kj} \mathbf{z}_{kj}^{[s]}\, ,  \qquad \mathrm{(OMA)} \label{eq:oma_signal}
\end{equation}
%\begin{equation}
%    \mathbf{y}_{k}^{[s]} = w_k \sum_{j \in \mathcal{N}_k} h_{k}^{[s]} \mathbf{x}_k^{[s]} + \mathbf{z}_k^{[s]}  \qquad \mathrm{(NOMA)} 
%end{equation}
where $h_{kj}^{[s]}$ is the channel gain between agent $k$ and $j$ in round $s$, $\mathbf{x}_{j}^{[s]}$ is an uncoded function of the \textcolor{black}{local samples $\boldsymbol\theta_j^{[s]}$}
\begin{equation}
    \mathbf{x}_j = \alpha_{kj}^{[s]} \boldsymbol\theta_{j}^{[s]}
\end{equation}
with some parameters $\alpha_{kj}^{[s]}$, 
%and $\mathbf{z}_{kj}^{[s]} \sim \mathcal{N}(0, N_0 \mathbf{I}_{m})$ is the Gaussian i.i.d. channel noise.  
%\textcolor{red}{To simplify the analysis, we consider that the channel coefficients and the noise among devices depends only on the transmitting device, namely $h_{jk}^{[s]} = h_{j}^{[s]}$ and $\mathbf{z}_{kj}^{[s]} = \mathbf{z}_{j}^{[s]}$ in \eqref{eq:oma_signal}.}
Each agent $k$ employs the following uncoded function for transmitting the samples to its neighbors 
\begin{equation}
    \label{eq:uncoded_function}
    \mathbf{x}_k^{[s]} = \alpha_{kj}^{[s]} \boldsymbol\theta_{k}^{[s]} \, , 
\end{equation}
where $\alpha_{kj}^{[s]}$ is a power control parameter. 
%The encoded functions are implemented by considering the truncated channel inversion as 
%\begin{equation}
%    \alpha_{kj}^{[s]} = 
%    \begin{cases}
%    \alpha^{[s]}/h_{kj}^{[s]}, &  \mathrm{if} \, |h_{kj}^{[s]}| \geq g^{[s]}, \\
%    0,  & \mathrm{if} \, |h_{kj}^{[s]}| < g^{[s]} \, , 
%    \end{cases}
%    \label{eq:channel_inversion_oma}
%\end{equation}
%where $\alpha^{[s]}$ and $g^{[s]}$ are parameters to be optimized. taking into account the power constraint of the devices $\| \mathbf{x}_{j}^{[s]}\|^{2} \leq P$. 
%Thus, device $k$ transmits its samples only if its channel is large enough, namely $|h_k^{[s]}| \geq g^{[s]}$.
Considering NOMA, the agents exploit exploit over-the-air computing to aggregate the samples received from their neighbors, leading to the following received signal
%Agents may also employ over-the-air computing to aggregate the samples received from their neighbors via non-orthogonal multiple access (NOMA). 
%In this case, the received signal can be expressed as 
\begin{equation}
    \mathbf{y}_k^{[s]} = \sum_{j \in \mathcal{N}_{k}} h_j^{[s]} \mathbf{x}_k^{[s]} +  \mathbf{z}_k^{[s]}\, ,  \qquad \mathrm{(NOMA)} \label{eq:noma_signal}
\end{equation}
where $h_j^{[s]}$ is the channel coefficient and $\mathbf{z}_k^{[s]} \sim \mathcal{N}(0, \mathbf{I}_m)$ is a i.i.d. Gaussian noise. 
The encoded functions are implemented as
\begin{equation}
    \alpha_k^{[s]} = 
    \begin{cases}
    \alpha^{[s]} w_{kj} /h_{j}^{[s]} , &  \mathrm{if} \, |h_k^{[s]}| \geq g^{[s]}\, , \\
    0,  & \mathrm{if} \, |h_k^{[s]}| < g^{[s]} \, , 
    \end{cases}
    \label{eq:channel_inversion_noma}
\end{equation}
where, $\alpha^{[s]}$ and $g^{[s]}$ are parameters to be optimized under the power constraint of the devices $\| \mathbf{x}_{j}^{[s]}\|^{2} \leq P$. 
%Given the channel coefficients, the agents implement truncated channel inversion whereby the power control parameter is selected as 
%\begin{equation}
%    \alpha_k^{[s]} = 
%    \begin{cases}
%    \alpha^{[s]}/h_k^{[s]}, &  \mathrm{if} \, |h_k^{[s]} \geq g^{[s]}, \\
%    0,  & \mathrm{if} \, |h_k^{[s]} < g^{[s]} 
%    \end{cases}
%    \label{eq:channel_inversion}
%\end{equation}
%where $\alpha^{[s]}$ and $g^{[s]}$ are parameters to be optimized. taking into account the power constraint of the devices $\| \mathbf{x}_{j}^{[s]}\|^{2} \leq P$. 
%The agents must also satisfy a transmit power constraint $\| \mathbf{x}_{j}^{[s]}\|^{2} \leq P$. 

\subsection{Scheduling strategy and D-SGLD update}

We adopt the scheduling strategy proposed in [ADD REF] and compute the D-SGLD update as follows.
All devices $i \in \mathcal{V}$ scheduled in a slot $s \in \mathcal{S}_{i}^{AT} \bigcap \mathcal{S}_i^{AR}$ transmit their samples simultaneously to enable \textit{AirComp} aggregation at a central node $j$ by pre-compensating their channels as
\begin{equation}
    \mathbf{x}_{ij}^{[s, t_s]} = \dfrac{\sqrt{\gamma_j^{[t,s]}}}{h^{'}_{ij}} w_{ij} \boldsymbol\theta_i^{[s]}
\end{equation}
where $\gamma_j^{[t,s]}$ is a power scaling factor for channel alignment at device $j$. The central node $j$ receives the superposition of the transmitted signals
\begin{equation}
    \mathbf{y}_{j}^{[s, t_s]} = \sqrt{\gamma_j^{[s, t_s]}} \sum_{i \in \mathcal{N}_j^{(t_s)}} w_{ij} \boldsymbol\theta_i^{[s]} +  \mathbf{n}_{j}^{[s, t_s]}
\end{equation}
and compensates for the power scaling factor to obtain the following estimate of the received signals
\begin{equation}
    \hat{\mathbf{y}}_{j}^{[s, t_s]} = \dfrac{\mathbf{y}_j^{[s, t_s]}}{\sqrt{\gamma_j^{[s, t_s]}}} = \sum_{i \in \mathcal{N}_{j}^{(t_s)}} w_{ij} \boldsymbol\theta_i^{[s]} + \dfrac{\mathbf{n}_{j}^{[s, t_s]}}{\sqrt{\gamma_j^{[s, t_s]}}} \, .
\end{equation}
Next, the devices $i \in \mathcal{V}$ scheduled in the slot $s \in \mathcal{S}^{BT}$ broadcast their samples to their immediate neighbors $j \in \mathcal{N}_i^{(t_s)}$ as
\begin{equation}
    \mathbf{x}_i^{[s, t_s]} = \sqrt{\alpha_i^{[s, t_s]}} \boldsymbol\theta_i^{[s]}
\end{equation}
where $\alpha_i^{[s, t_s]}$ is a transmitting power scaling factor. 
Thus, the received signal at each neighbor in slot $s \in \mathcal{S}_j^{BR}$ is
\begin{equation}
    \mathbf{y}_{ij}^{[s, t_s]} = \sqrt{\alpha_i^{[s, t_s]}} h_{ij}^{' (t)} \boldsymbol\theta_i^{[s]} + \mathbf{n}_j^{[s, t_s]} \, .
\end{equation}
Device $j$ estimates the signal as
\begin{equation}
    \hat{\mathbf{y}}_{ij}^{[s, t_s]} = \dfrac{ w_{ji} \mathbf{y}_{ij}^{[s, t_s}}{\sqrt{\alpha_i^{[s, t_s}} h_{ij}^{' (s)}} = w_{ji} \boldsymbol\theta_i^{[s]} + w_{ji} \dfrac{\mathbf{n}_j^{[s, t_s]}}{\sqrt{\alpha_i^{[s, t_s]}} h_{ij}^{' (s)}} \, .
\end{equation}
Upon completing the \textit{AirComp} and broadcast phase for all slots $s \in \mathcal{S}$, device $j \in \mathcal{V}$ updates its samples combining all samples received in the slots $s \in \mathcal{S}_j^{Rx} = \mathcal{S}_j^{BR} \bigcup \mathcal{S}_{j}^{AR}$ as
\begin{equation}
 \boldsymbol\theta_j^{[s + 1]} = w_{jj} \boldsymbol\theta_j^{[s]} + \sum_{s \in \mathcal{S}_{j}^{AR}} \hat{\mathbf{y}}_{j}^{[s, t_s]} + \sum_{s \in \mathcal{S}_{j}^{BR}} \hat{\mathbf{y}}_{i_{s} j}^{[s, t_s]} + ....
\end{equation}
where $i_s \in \mathcal{N}_j$ denotes the node transmitting in broadcast mode in slot $s \in \mathcal{S}_{j}^{BR}$.
Expanding the last equation we obtain
\begin{align}
   \boldsymbol\theta_j^{[s + 1]} &=   w_{jj} \boldsymbol\theta_j^{[s]} + \sum_{s \in \mathcal{S}_{j}^{AR}} \hat{\mathbf{y}}_{j}^{[s, t_s]} + \sum_{s \in \mathcal{S}_{j}^{BR}} \hat{\mathbf{y}}_{i_{s} j}^{[s, t_s]} + .... \\
   &=  w_{jj} \boldsymbol\theta_j^{[s]} + \sum_{s \in \mathcal{S}_{j}^{AR}} \left[ \sum_{i \in \mathcal{N}_{j}^{(t_s)}} w_{ij} \boldsymbol\theta_i^{[s]} + \dfrac{\mathbf{n}_{j}^{[s, t_s]}}{\sqrt{\gamma_j^{[s, t_s]}}} \right] + \sum_{s \in \mathcal{S}_{j}^{BR}} \left[ w_{ij} \boldsymbol\theta_i^{[s]} + \dfrac{w_{ij} \mathbf{n}_j^{[s, t_s]}}{\sqrt{\alpha_i^{[s, t_s]}} h_{ij}^{' (s)}} \right] \\
   &= w_{jj} \boldsymbol\theta_j^{[s]} + \sum_{s \in \mathcal{S}_{j}^{AR}}  \sum_{i \in \mathcal{N}_{j}^{(t_s)}} w_{ij} \boldsymbol\theta_i^{[s]} + \sum_{s \in \mathcal{S}_{j}^{AR}}  \sum_{i \in \mathcal{N}_{j}^{(t_s)}} \dfrac{\mathbf{n}_{j}^{[s, t_s]}}{\sqrt{\gamma_j^{[s, t_s]}}} +  \sum_{s \in \mathcal{S}_{j}^{BR}} w_{ij} \boldsymbol\theta_i^{[s]} + \sum_{s \in \mathcal{S}_{j}^{BR}}\dfrac{w_{ij} \mathbf{n}_j^{[s, t_s]}}{\sqrt{\alpha_i^{[s, t_s]}} h_{ij}^{' (s)}} \\
   &= w_{jj} \boldsymbol\theta_j^{[s]} + \sum_{s \in \mathcal{S}_{j}^{AR}}  \sum_{i \in \mathcal{N}_{j}^{(t_s)}} w_{ij} \boldsymbol\theta_i^{[s]} +  \sum_{s \in \mathcal{S}_{j}^{BR}} w_{ij} \boldsymbol\theta_i^{[s]} + \sum_{s \in \mathcal{S}_{j}^{AR}}  \sum_{i \in \mathcal{N}_{j}^{(t_s)}} \dfrac{\mathbf{n}_{j}^{[s, t_s]}}{\sqrt{\gamma_j^{[s, t_s]}}} + \sum_{s \in \mathcal{S}_{j}^{BR}}\dfrac{w_{ij} \mathbf{n}_j^{[s, t_s]}}{\sqrt{\alpha_i^{[s, t_s]}} h_{ij}^{' (s)}} \\
   &= \sum_{i \in \mathcal{N}_{j} \bigcup \{j\}} w_{ij} \boldsymbol\theta_i^{[s]} + \underbrace{\sum_{s \in \mathcal{S}_{j}^{AR}}  \sum_{i \in \mathcal{N}_{j}^{(t_s)}} \dfrac{\mathbf{n}_{j}^{[s, t_s]}}{\sqrt{\gamma_j^{[s, t_s]}}} + \sum_{s \in \mathcal{S}_{j}^{BR}}\dfrac{w_{ij} \mathbf{n}_j^{[s, t_s]}}{\sqrt{\alpha_i^{[s, t_s]}} h_{ij}^{' (s)}}}_{\mathrm{effective \, noise \, for \, sampling}}
\end{align}
Thus, to obtain a valid \ac{d-sgld} update, one should constrain that the overall injected noise from the channel to have variance no more than $2 \eta$.
In other words, 
\begin{equation}
    \mathrm{Var} \left(\sum_{s \in \mathcal{S}_{j}^{AR}}  \sum_{i \in \mathcal{N}_{j}^{(t_s)}} \dfrac{\mathbf{n}_{j}^{[s, t_s]}}{\sqrt{\gamma_j^{[s, t_s]}}} + \sum_{s \in \mathcal{S}_{j}^{BR}}\dfrac{w_{ij} \mathbf{n}_j^{[s, t_s]}}{\sqrt{\alpha_i^{[s, t_s]}} h_{ij}^{' (s)}} \right) = 2 \eta
\end{equation}
\begin{equation}
    N_0 \left[ \left( \sum_{s \in \mathcal{S}_{j}^{AR}}  \sum_{i \in \mathcal{N}_{j}^{(t_s)}} \dfrac{1}{\sqrt{\gamma_j^{[s, t_s]}}} \right)^2 +  \left( \sum_{s \in \mathcal{S}_{j}^{BR}}\dfrac{w_{ij} }{\sqrt{\alpha_i^{[s, t_s]}} h_{ij}^{' (s)}} \right)^2 \right] = 2 \eta
\end{equation}
\begin{equation}
    N_0 \left( \sum_{s \in \mathcal{S}_{j}^{AR}}  \sum_{i \in \mathcal{N}_{j}^{(t_s)}} \dfrac{1}{\sqrt{\gamma_j^{[s, t_s]}}} \right)^2 + \dfrac{N_0 w_{ij}^2 |S_j^{BR}|}{\alpha_i^{[s, t_s]} h_{ij}^{' [s]}} = 2 \eta
\end{equation}

==> sections/lidar_classification.tex <==
\section{numerical results}
